FlexPose: Pose Distribution Adaptation with Limited Guidance

Numerous well-annotated human key-point datasets are publicly available to date. However, annotating human poses for newly collected images is still a costly and time-consuming progress. Pose distributions from different datasets share similar pose hinge-structure priors with different geometric transformations, such as pivot orientation, joint rotation, and bone length ratio. The difference between Pose distributions is essentially the difference between the transformation distributions. Inspired by this fact, we propose a method to calibrate a pre-trained pose generator in which the pose prior has already been learned to an adapted one following a new pose distribution. We treat the representation of human pose joint coordinates as skeleton image and transfer a pre-trained pose annotation generator with only a few annotation guidance. By fine-tuning a limited number of linear layers that closely related to the pose transformation, the adapted generator is able to produce any number of pose annotations that are similar to the target poses. We evaluate our proposed method, FlexPose, on several cross-dataset settings both qualitatively and quantitatively, which demonstrates that our approach achieves state-of-the-art performance compared to the existing generative-model-based transfer learning methods when given limited annotation guidance.

==> Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := main

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex


clean:
	rm -f *.log *.aux *.blg *.bbl *.gz *.dvi \
		*.thm *.dat *.out *.run.xml *.bcf *.data


==> setting-aaai.tex <==
% =============================================================
%         Setting for AAAI format
%
%   Author      : Bei Yu
%   Last Update : 07/2023
% =============================================================


\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{bbm} % forbidden by aaai
\usepackage[hyphens]{url}
\usepackage{url}
\usepackage[table]{xcolor}
\usepackage{cleveref}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\usepackage{threeparttable,booktabs}
\usepackage{makecell}
\usepackage{multirow}
\usepackage[]{algpseudocode}                               % algorithm package
%\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{courier}
\usepackage[inline]{enumitem}
\usepackage{tabularx}
\usepackage{soul}
\usepackage{bm}
\usepackage{pifont}                                        % add circle
\usepackage{bbding}                                        % Checkmark
\usepackage[super]{nth}

\newcommand{\minisection}[1]{\noindent{\textbf{#1}}}
\newcommand{\minienumerate}[1]{\noindent{\textbf{#1}}}
\newcommand{\tabincell}[2]{
    \begin{tabular}{@{}#1@{}}#2\end{tabular}
}


% === Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\tensor}[1]{\boldsymbol{\mathcal{#1}} }    % tensor 
\renewcommand{\vec}[1]{\boldsymbol{#1}}                % re-define vec command
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\mathbbm}[1]{\text{\usefont{U}{bbm}{m}{n}#1}}

% === Theorem Definitions
\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{myassumption}{\textbf{Assumption}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mycorollary}{\textbf{Corollary}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myexample}{\textbf{Example}}
\newtheorem{myconjecture}{Conjecture}
\newtheorem{myprop}{Property}
\newtheorem{remark}{Remark}[section]

% === shrink page num
\setlength{\textfloatsep}{8pt plus 1pt minus 1pt}         % set space between float and text
\setlength{\floatsep}{10pt plus 1pt minus 1pt}             % set space between two floats
\setlength{\intextsep}{6pt plus 1pt minus 1pt}             % set space between text and float
\setlength{\belowdisplayskip}{4pt} \setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}



